Applying the causal roadmap to longitudinal national Danish registry data: a case study of second-line diabetes medication and dementia

The causal roadmap is a formal framework for causal and statistical inference that supports clear specification of the causal question, interpretable and transparent statement of required causal assumptions, robust inference, and optimal precision. The roadmap is thus particularly well-suited to evaluating longitudinal causal effects using large scale registries; however, application of the roadmap to registry data also introduces particular challenges. In this paper we provide a detailed case study of the longitudinal causal roadmap applied to the Danish National Registry to evaluate the comparative effectiveness of second-line diabetes drugs on dementia risk. Specifically, we evaluate the difference in counterfactual five-year cumulative risk of dementia if a target population of adults with type 2 diabetes had initiated and remained on GLP-1 receptor agonists (a second-line diabetes drug) compared to a range of active comparator protocols. Time-dependent confounding is accounted for through use of the iterated conditional expectation representation of the longitudinal g-formula as a statistical estimand. Statistical estimation uses longitudinal targeted maximum likelihood, incorporating machine learning. We provide practical guidance on the implementation of the roadmap using registry data, and highlight how rare exposures and outcomes over long-term follow up can raise challenges for flexible and robust estimators, even in the context of the large sample sizes provided by the registry. We demonstrate how simulations can be used to help address these challenges by supporting careful estimator pre-specification. We find a protective effect of GLP-1RAs compared to some but not all other second-line treatments.

==> archive/archive_body.tex <==
\section{Introduction}\label{sec1}

There has been a significant increase in the amount of existing observational or``real world’’ health data both collected by and aggregated for researchers over the past few decades. This type of data has become increasingly important in medical decision-making, as it allows researchers to answer questions that would not be feasible in a prospective trial due to treatment guidelines, financial constraints, ethical considerations, or logistical challenges. Electronic health record databases, with their large sample sizes and long follow-up times, enable the study of rare outcomes, realistic treatment usage, and more generalizable populations. However, because observational data are particularly susceptible to unobserved confounding and selection bias, real-world evidence is often used only for associational analyses and causal claims are discouraged. \cite{hernan_c-word_2018,parra_consistency_2021,amastyleinsider_use_2017} Further, standard statistical estimation approaches that rely on pre-specified parametric models may fail to fully adjust for even measured confounders available in registries, while ad hoc model adaptation based on data exploration undercuts the basis of robust statistical inference. 

The causal roadmap provides a structured framework for navigating these challenges and generating robust evidence for causal questions.\cite{petersen_causal_2014}  Specifically, the causal roadmap provides guidance for the following steps: 1) translation of a causal question, such as the comparative effectiveness of two longitudinal treatment protocols, into a formally defined \emph{causal estimand}; 2) explicit statement of the \emph{observed data} and knowledge about the processes that gave rise to it (\emph{causal model})  3) \emph{identification}, or the formal translation of the causal estimand (which describes an ideal hypothetical experiment) into a \emph{statistical estimand} (a function of the observed data distribution that can be estimated) under explicit causal assumptions;  4) specification of a \emph{statistical model} that avoids any unsubstantiated statistical assumptions, and a \emph{statistical estimator} selected to provide the best expected performance (eg. nominal 95\% CI coverage, minimum variance); and, 5) support for \emph{interpretation} in the context of these assumptions, including sensitivity analyses.

Large, comprehensive, and representative longitudinal datasets those of national registries offer advantages for evaluating causal effects; they allow for generalizable study populations and investigation of the real-world effectiveness of long term treatments on rare outcomes. Their use also introduces challenges by making implementation of the full casual roadmap simultaneously more complex and arguably even more essential to ensure robust inferences. The full longitudinal counterfactual interventions of interest must be specified, including not only initial treatment assignments, but also any post baseline restrictions on treatment modification or drop-in, as well as any hypothetical interventions on treatment compliance, censoring or measurement. \cite{petersen_applying_2014} Specification of a ``target trial’’\cite{hernan_using_2016}  is one commonly used device to support specification of a causal estimand; however, specification of post-baseline ``interventions’’ or protocols, including those to enforce compliance or to prevent censoring, need not correspond to any realistic intervention that might be accomplished in an actual trial. 

Both the observed data and confounding structures in longitudinal registry data are complex, and thus identification of the target causal estimand in such studies requires a more complex statistical estimand, such as the longitudinal g formula.\cite{laan_targeted_2018} This in turn necessitates more complex statistical estimation capable of adjusting for time-varying confounders. Many of the advantages of using registry data---including the ability to study the effects of prolonged treatments on rare outcomes and capture of a wide range of potential and time-dependent confounders---also introduce additional challenges to estimation. Flexible machine learning approaches to covariate adjustment are paramount to make optimal use of complex longitudinal data captured in a registry; but must be implemented such that statistical inference is preserved.\cite{ laan_targeted_2018} Further, even with initially large sample sizes and common treatments, the number of persons who comply with long term protocols can dwindle quickly, resulting in practical positivity violations. Finally, the unique ability of registries to evaluate effects on rare and unbalanced outcomes can introduce new challenges to estimator performance. Careful estimator specification and benchmarking can address many of these challenges; however, in order to provide a firm basis for statistical inference, the full estimation procedure must be pre-specified.

Motivated by both the utility of full application of the causal roadmap to longitudinal registry analyses, and the practical challenges that arise in its application, in this paper we present a detailed case study of the use of the longitudinal roadmap to evaluate the long term cumulative causal effect of second-line diabetes medications on dementia risk among a cohort of diabetes patients using the Danish National Registry. The Danish National registry is one of the longest-standing national registry databases that has expansive longitudinal data dating back several decades.\cite{schmidt_danish_2015} Due to its large size, rich covariate measurement and long follow up, the Danish registry is well-suited for examining rare and longer-term exposures and outcomes. It also has a high degree of diagnostic reliability for some but not all diseases, with a positive predictive value of 0.96 and 0.98 for diabetes and dementia, respectively.\cite{thygesen_predictive_2011}  Dementia affects around three percent of the older Danish population, but several studies suggest the true prevalence is higher.\cite{noauthor_dementia_nodate-1}  Dementia is particularly burdensome to the diabetic population. \cite{biessels_risk_2006} While newer second-line diabetes medications may hold promise in preventing neurodegeneration, many of these medications are relatively rare in the diabetes populations. Due to the rare nature of both exposure and outcome of interest, examining this relationship without the use of a large data source like the Danish registry would be infeasible.

With this motivation, we evaluate the difference in counterfactual five-year cumulative risk of dementia if a target population of adults with type 2 diabetes had initiated and remained on GLP-1 agonists, a new class of drugs, compared to a range of active comparator protocols. Time-dependent confounding is accounted for through use of the iterated conditional expectation estimator of the longitudinal g-formula as statistical estimand.\cite{bang_doubly_2005,wen_parametric_2021}  Statistical estimation is conducted in a fully non-parametric model, and uses longitudinal targeted maximum likelihood estimation, incorporating machine learning, in order to flexibly incorporate covariate adjustment. Our case study provides practical guidance on the implementation fo the roadmap in large scale registry data. In particular, we highlight how rare and unbalanced outcomes can raise challenges for flexible and robust estimators such as TMLE even in the context of the large sample sizes provided by the registry and discuss estimation approaches to addressing these challenges, including careful specification of the machine learning library and selection of an appropriate variance estimator. We show how outcome-blind simulations can be used inform to pre-specification of these important decisions (a prerequisite for valid statistical inference) in order to optimize the expected performance of the statistical estimator (in terms of confidence interval coverage and precision). As we discuss, simulations can also be useful in the case of registry data that can be difficult to access for logistical reasons, prompting further need for simulated data.

There are examples of previous analyses of Nordic registry data using a target trial framework. \cite{olarte_parra_trial_2022,rossides_infection_2021} However, these analyses do not follow a causal roadmap, and consequently conflate the target causal parameter of interest and statistical estimation. For example, censoring is often conceptualized as a statistical estimation problem rather than a part of the intervention of interest. \cite{olarte_parra_trial_2022} Studies also tend to employ a hazard ratio, which is difficult to interpret causally \cite{hernan_hazards_2010}. There are examples of longitudinal applied roadmap analyses that make this explicit\cite{ montoya_estimators_2022,tran_evaluating_2016} , but these have not been implemented at the scale on national registry data. This is the first study to apply the causal roadmap to a national registry of over 300,000 diabetes patients.\cite{international_diabetes_federation_denmark_nodate}  

This paper is organized as follows: in section 2, we step through application of the causal roadmap to our case study, evaluating the long-term effect of GLP-1 RA use on incident dementia risk using the Danish National Registry, up to the step of statistical estimation. We  illustrate opportunities, challenges, and practical responses at each step of the roadmap. In Section 3, we specify the statistical model and detail the estimation procedure, including simulation and analysis plan. In particular, we provide a detailed overview of key estimation choices in the implementation of our longitudinal targeted maximum likelihood estimator, and the use of simulations to guide these choices. In Section 4, we present the results and interpretation of our analysis, including sensitivity analyses. In section 5, we discuss the findings and the implications of this work.

%There has been a significant increase in the amount of observational or ``real-world'' health data both collected and aggregated for researchers over the past few decades. This type of data has become increasingly important in medical decision-making, as it allows researchers to answer questions that would not be feasible in a prospective trial due to treatment guidelines, financial constraints, ethical considerations, or logistical challenges. Electronic health record databases, with their large sample sizes and long follow-up times, enable the study of rare outcomes, realistic treatment usage, and more generalizable populations. However, because observational data are particularly susceptible to unobserved confounding and selection biasreal-world evidence is often used only for associational analyses and causal claims are discouraged.\cite{hernan_c-word_2018,parra_consistency_2021,amastyleinsider_use_2017}, 

%Causal inference is a framework for drawing valid causal conclusions from data, including observational data. The causal roadmap is a tool that helps integrate causal thinking into applied research by guiding researchers to: frame causal questions; transparently state and evaluate the plausibility of assumptions required for causal inference; define the potential gap between statistical estimation and the target parameter of interest; and interpret the results in the context of these assumptions.\cite{petersen_causal_2014} The longitudinal causal roadmap applies these guidelines to time-varying data, and allows for clear specification of a longitudinal counterfactual treatment of interest, including the intervention on treatment compliance and censoring or measurement.\cite{petersen_applying_2014,hernan_hazards_2010} As part of this roadmap, researchers must define their causal quantities of interest. This is often done in terms of a hypothetical target trial.\cite{hernan_using_2016} The target trial framework provides clarity in the analytic goals of observational research, especially to a clinical audience. In addition to specifying an ideal trial, however, it is important to detail the full intervention on the structural causal model, including elements not realistic to intervene on in a trial, such as loss to follow-up and non-compliance.

%It is also key to select a measure of effect appropriate for the longitudinal analysis. In medical research, the hazard ratio is commonly used. A hazard is the instantaneous rate of having an event, given that the event has not already occurred. At each time point, the hazard ratio thus compares event rates between study arms among participants who remain event-free. Over time, this measure is susceptible to an inherent selection bias. For example, if the treatment is detrimental early in follow-up, individuals who remain event-free in the treatment arm will soon be at lower risk than individuals who remain event-free in the control arm. Susceptibility to the outcome is thus no longer balanced between arms; the treatment arm is instead at an inherent advantage. It becomes impossible to recover a counterfactual quantity generally of interest in a causal study using the hazard ratio. 
%advantages of registry- more complex causal estimands are feasible but this raises challenges] 

%Target trials are best implemented on large and comprehensive, representative datasets as they allow for narrower target trial inclusion criteria while maintaining a large sample size and a generalizable study sample. The Danish National registry is one of the longest-standing national registry databases that has expansive longitudinal data dating back several decades.\cite{schmidt_danish_2015} Due to its large size, rich covariate measurement and long follow up, the Danish registry is well-suited for examining rare and longer-term exposures and outcomes. It also has a high degree of diagnostic reliability for some but not all diseases, with a positive predictive value of 0.96 and 0.98 for diabetes and dementia, respectively.\cite{thygesen_predictive_2011}

%In this study, we examine the longitudinal causal effect of second-line diabetes medications on dementia risk among a cohort of diabetes patients. Dementia affects around three percent of the older Danish population, but several studies suggest the true prevalence is higher.\cite{noauthor_dementia_nodate-1} Dementia is particularly burdensome to the diabetic population. While newer second-line diabetes medications may hold promise in preventing neurodegeneration, many of these medications are relatively rare in the diabetes populations. Due to the rare nature of both exposure and outcome of interest, examining this relationship without the use of a large data source like the Danish registry would be infeasible. 

%However, in part because of the advantages of registries (handling rare exposures/outcomes, longer-term follow up), estimation can be particularly challenging. High administrative censoring and uncommon treatments can result in violations of the positivity assumption (section 4.1). Many choices are made in estimating the causal quantity, and it is challenging to know how to optimally estimate target causal parameters under these challenges. Outcome-blind simulations allow you to pre-specify these decisions in a thoughtful way. They allow you to choose the more efficient estimator while avoiding `p-hacking'\cite{ioannidis_why_2005} or selective reporting of results. Simulations also help to prevent overfitting by allowing researchers to choose the best estimation procedure among several candidates. This can also be useful in the case of registry data that can be difficult to access for logistical reasons.

%There are examples of previous analyses of Nordic registry data using a target trial framework.\cite{olarte_parra_trial_2022,rossides_infection_2021} However, these analyses do not follow a causal roadmap, and consequently conflate the target causal parameter of interest and statistical estimation. In the case of a Swedish study of renal disease, for example, censoring was conceptualized as a statistical estimation problem rather than a part of the intervention of interest.\cite{olarte_parra_trial_2022} 
%The study also employs a hazard ratio, a common measure used in prospective clinical studies that suffers from the aforementioned selection bias. There are examples of longitudinal applied roadmap analyses that make this explicit \cite{tran_evaluating_2016, montoya_estimators_2022} but not at scale on registry data. This is the first study to apply the causal roadmap to a national registry of over 300,000 diabetes patients.\cite{international_diabetes_federation_denmark_nodate} We also integrate applied simulations into the roadmap for pre-specifying estimation, including the use of machine learning to estimate a double-robust estimator.

%This paper is organized as follows: in section 2, we introduce the case study. In section 3, we describe the causal question and observed data structure. In Section 4, we outline the target causal parameters of interest and identification assumptions. In Section 5, we detail the estimation procedure, including simulation and analysis plan. In Section 6, we review the study population, simulation results, and main results. In section 7, we discuss the findings and the implications of this work.

\section{Case study of the longitudinal causal roadmap: evaluating the long term effect of GLP-1RA use on incident dementia risk using the the Danish National Registry}
\subsection{Background and motivation}

Type two diabetes mellitus (T2DM) is a cardio-metabolic disease that affected 462 million people globally in 2017, and is increasing in prevalence each year.\cite{khan_epidemiology_2020}  It characterized by elevated blood sugar levels which over time can strain not only the cardiovascular but also the nervous system.\cite{cdc_what_2020} T2DM has been shown to accelerate brain aging and neurodegeneration that are antecedent to dementia.\cite{umegaki_type_2014,biessels_risk_2006} Dementia is a progressive neurodegenerative disease characterized by impaired cognitive functioning that interferes with daily life. While the exact mechanisms are an active area of research, diabetes generally hastens neurodegeneration and resulting the pathways through a complex mixture of defective insulin signaling, metabolic/mitochondrial dysfunction, oxidative stress, and vascular damage, among others.\cite{tumminia_type_2018, duarte_crosstalk_2013}

The connection between GLP-1RAs and improved cognition has been well-demonstrated in mouse models. Specifically, liraglutide (a GLP-1RA) reduced neuroinflammation and improved synaptic function (reducing amaloyoid formation).\cite{mcclean_diabetes_2011,mcclean_glucagon-like_2010} GLP-1RAs are thought to be particularly protective both because of their effects on glucose regulation (and subsequently weight reduction) as well as a direct effect on neuroplasticity.\cite{duarte_crosstalk_2013,boye_generalizability_2019, onoviran_effects_2019} Secondary analyses of randomized placebo-controlled trial data in diabetic patients also showed a significant reduction in cognitive decline among those in the GLP-1RA treatment arm compared to control arm.\cite{vadini_liraglutide_2020, ballard_liraglutide_2020,biessels_effect_2019} Due to the short-term follow up of these randomized studies, the outcome of interest was either cognitive worsening (from validated cognition tests) or dementia-related adverse events. Studying dementia onset requires longer-term follow up seldom practically or financially feasible for most randomized trials. Trial participants in these secondary analyses were also higher risk and not representative of the general population.

Observational studies circumvent these shortcomings by allowing access to expansive datasets with sufficient number of events to look at relatively rare exposures or outcomes and evaluate long-term treatment effects. A growing body of observational research studying the effects of GLP-1RAs on dementia has shown a reduction in dementia risk.\cite{norgaard_treatment_2022,wium-andersen_antidiabetic_2019,ballard_liraglutide_2020} In the Danish National Registry specifically, one analysis showed a protective effect of GLP-1RA use on dementia for every year increase in exposure.\cite{norgaard_treatment_2022} While these results are encouraging, application of the causal roadmap illustrates how they may fall short of estimating the causal effect of greatest interest. (1)\emph{Causal estimand specification}: some used a hazard ratio to measure effect\cite{ballard_liraglutide_2020,norgaard_treatment_2022}; while commonly used, the hazard ratio not easily causally interpretable. A hazard is the instantaneous rate of having an event given that the event has not already occurred, and thus at each time point the hazard ratio compares event rates between study arms among participants who remain event-free. By definition, over time, this measure is susceptible to an inherent selection bias which can make it impossible to recover a counterfactual quantity generally of interest in a causal study.\cite{hernan_hazards_2010} (2)\emph{Identificiation}: in order to causally interpret results, we must satisfy the sequential randomization assumption (see Section 2.3.1), which states that the counterfactual outcome must be independent of treatment assignment, conditional on measured past. Adjusting for only baseline covariates (as done in a Cox proportional hazards model) may not be sufficient to adjust for confounding, particularly if there are time-dependent confounders that are affected by past treatment usage and affect future treatment usage. 
%(3) \emph{Estimation}:

%For example, if the treatmentis detrimental early in follow-up, individuals who remain event-free in the%treatment arm will soon be at lower risk than individuals who remain event-freein the control arm. Susceptibility to the outcome is thus no longer balanced betweenarms; the treatment arm is instead at an inherent advantage. 


%\subsection{Causal question}
Through the  subsequent analysis, we seek apply the longitudinal causal roadmap to answer the question: what is the effect of sustained, cumulative exposure to GLP-1RAs vs i) any active comparator or, ii) specific active comparators (Sodium-glucose Cotransporter-2 or SGLT2 Inhibitors, Dipeptidyl peptidase 4 or DPP-4 inhibitors) on the cumulative risk of dementia by 5 years among patients with T2DM initiating second-line antihyperglycemic therapy for the first time? For each of these causal questions, in this section we outline the causal estimand, specify the observed data and a causal model describing what is known about the real-world processes that generated it, and finally identify the causal estimand as a statstical estimand---a function of the observed data distribution that can be, and that is equivalent to the causal estimand under explicit causal assumptions. This sets the stage for defining the statistical estimation problem and specifying an estimator, as we do in the subsequent section.


\subsection{Causal estimand}
We define two target causal parameters of interest for the purposes of this analysis: one intervening only on the exposure of interest (use of GLP-1RAs, $A_1 (t)$) and censoring ($C(t)$), and the other intervening additionally on  an active comparator of interest ($A_2 (t)$).
%\subsection{Treatment regimes of interest}
Our counterfactual outcomes of interest  when intervening only on GLP-1RA use $A_1$ correspond to the time to diagnosis of dementia that would have been seen under these two hypothetical regimes (Table 1):
$$Y_{\bar{a}_1=1, c=0}(t),Y_{\bar{a}_1=0, c=0}(t), t=1,...,K+1 $$

Our counterfactual outcomes of interest  when intervening on both exposure $A_1$ and an active comparator $A_2$ correspond to the time to diagnosis of dementia that would have been seen under these two hypothetical regimes (Table 1):
$$Y_{\bar{a}_1=1,\bar{a}_2=0, c=0}(t),Y_{\bar{a}_1=0,\bar{a}_2=1, c=0}(t), t=1,...,K+1 $$
%\subsection{Target causal parameters}
In our first target parameter, we are interested in the cumulative causal risk difference for dementia diagnosis  up to the maximum of follow up time if all patients had complied with the intervention arm vs. the control arm, intervening to prevent administrative censoring (Table 1):
$$E[Y_{\bar{a}_1=1, c=0}]-E[Y_{\bar{a}_1=0, c=0}]$$

In our second target causal parameter, we additionally intervene on an active comparator:
$$E[Y_{\bar{a}_1=1,\bar{a}_2=0, c=0}]-E[Y_{\bar{a}_1=0,\bar{a}_2=1, c=0}]$$

Here, we are contrasting full GLP-1RA use, no active comparator use and no administrative censoring throughout follow up, compared to full active comparator use (eg. SGLT2), no GLP-1RA use and no administrative censoring throughout follow up.

\newpage
\begin{landscape}
\begin{table}[H]
\input{trial_table.tex}
\end{table}
\end{landscape}
\newpage
\subsection{Observed data and causal model}
We aggregated patient-level data a retrospective cohort of diabetes patients who met the following inclusion criteria: were at least 50 years of age; had evidence of prior metformin use; initiated a second line medication between 2009 and 2021 (second line start date as the index date); were insulin-naive and dementia-free at index date. (Supplemental Materials 1)

Data from this cohort can be described by a general longitudinal data structure, denoted as:

$$ O = (W, A(1), ..., L(K), A(K), L(K+1)) \sim  P_0$$
where W denotes baseline (time-invariant) covariate information, and $A(1)$ is exposure status at the beginning of the first node or time interval (i.e. index date). $A$ nodes also include an administrative censoring mechanism, C, which denotes censoring during the time interval. For ease of notation above, we refer to the treatment and censoring processes together as  $A(t)=(A_1(t), A_2(t), C(t))$. We refer to the covariate and outcome nodes collectively as $L(t)=(L(t), Y(t))$, which includes both time-varying covariate information $L(t)$ and outcome information $Y(t)$. Death will be considered a competing risk in the primary analyses and is thus also included in $L(t)$. Index date and baseline measurements are measured at the date of switch to second-line regimen. Here we use a 6-month time scale for time increments in the main analyses. $K+1$ is defined as the maximum follow up time. For notational convenience, we define variables after death, dementia diagnosis or censoring as equal to their last observed value. For further explanation of the data generating process, see Supplemental Materials 1. 

%\subsubsection{Exposure}
We utilized prescription fill data from the Danish registry to define exposure to diabetes medications. In the case of our medication exposure $A(t)$, we assume any medication fill as use of the medication for the following 6 months. We will consider two exposure nodes, $A_1(t)$ defined as exposure to GLP-1RAs at the beginning of the time period t, and $A_2(t)$, defined as exposure to an active comparator, however designated, at the beginning of time period t. For a full list of secondline diabetes medications used and relevant ATC codes, see Supplemental Materials 2.

%\subsubsection{Outcome Y(t): Dementia}
 We approximate  our outcome, dementia onset, by time $t$ through either of the following criteria:(1) dementia diagnosis, measured through inpatient diagnosis codes; or (2) purchase of dementia medication, measured through registry medication fill table. For a list of ICD and ATC codes used, see Supplemental Materials 2.
%\subsubsection{Covariates}
%For time-constant covariates, there was little to no missingness (\(\leq5\%\)), and we imputed to the median and mode for continuous and categorical covariates, respectively. 
We consider the following baseline covariates: age (years), sex (male/female), education (basic, some college, college or higher), baseline income (tertiles), time on metformin prior to index date (days). We also consider the following time-varying diagnosis covariates: heart failure, renal disease, chronic pulmonary disease, any malignancy, ischemic heart disease, myocardial infarction, hypertension, stroke. These covariates remain 0 until evidence of their presence through an inpatient ICD code in the registry is detected, then remain 1 for the remainder of follow up. We also included relevant medication use, including: beta-blockers, calcium channel blockers, renin-angiotensin system-acting inhibitors (RASI), loop diuretics, Mineralocorticoid receptor antagonists (MRAs) and COPD medications. For a more detailed definition of each covariate, see Supplemental Materials 3. Death is included in L(t), measured through the death records in the Danish registry. For each pairwise comparison, we adjust for other second-line medications not included in the contrast of interest, allowing them to vary naturally. 

\subsubsection{Identification: causal to statistical estimand}

The sequential randomization assumption posits that at each time point, the counterfactual outcome $Y$ is independent of treatment assignment, conditional on history of measured covariates and prior treatment:

$$ Y_{\bar{a}}\perp A(t) \mid  W, \bar{L}(t),\bar{A}(t-1)=\bar{a}(t-1), t=1,..,K$$

In other words, we must assume that in our causal model (Supplemental Materials 4), we have no unmeasured common causes of our `treatment decision' A at each time point and counterfactual outcome $Y_{\bar{a}}$ throughout follow up. In the case of GLP-1RA use, we must assume that at each time point t, a person's counterfactual outcome is independent of their treatment assignment at time t, conditional on their observed past.  For our second target causal parameter, intervening additionally on an active comparator, our counterfactual  outcome must be independent of treatment ($A_1$ and $A_2$) at each time point, conditional on the observable past. For each of these counterfactual outcomes at each time point, we need sufficient covariate information to control for any association between the counterfactual dementia endpoint and the treatment decision. Sequential randomization is an untestable assumption, though its feasibility is explored in the structural causal model outlined in Supplemental Materials 4. 

We must also assume we meet the positivity assumption, which states that there be a positive probability of treatment within each covariate stratum:
$$P(A(t)=a(t) \mid W=w,\bar{A-1}=\bar{a-1},\bar{L}=\bar{l}, t=1,...,K  \hspace{.5cm}   a.e. $$
We can verify this and address practical positivity violations prior to estimation. To address this, we explore treatment support in the results and in Supplemental Materials 5.


\section{Estimation}


\subsection{Simulation}
Simulations are a helpful tool that enable the selection of an optimally valid and efficient estimation procedure. Outcome-blind simulations allow for comparison of distinct estimation procedures while sill avoiding `p-hacking'. In the case of registry data that is not always easily accessible due to privacy concerns, simulations also allow researchers to work with realistic longitudinal data remotely where data is not available. Here, we use outcome-blind simulations to pre-specify our estimator, nuisance parameters (g and Q estimation), variance estimation, and handling of competing events. 

\subsubsection{Data generating process}
To simulate data with the complex longitudinal structure found in the Danish registry, we ran logistic regression models on the real registry cohort of interest (Section 5.1.1). We used these models to estimate each node at each time point, conditional on the observable past. We then created a matrix of beta coefficients from each of these regressions and exported them from the Danish server.

Using these coefficients, we simulated n=1000 (1) datasets of 115,698 observations with a significant relationship between exposure and outcome, and (2) equally-sized datasets with no relationship between exposure and outcome (``null data''). We simulated the datasets using the lava package.\cite{holst_linear_2013} For each node at each time point, we used the vector of beta coefficients to predict the node values. This dataset has a dependent correlation structure between exposure and outcome, reflective of the relationship in the true data. We then scrambled the outcome and censoring nodes in the dataset to create the null data (true risk difference of 0, true relative risk of 1). This allowed us to approximate the complex correlation structure of treatment and covariate measures in the data while remaining outcome-blind.

We estimated the true causal risk difference between full GLP-1RA use throughout follow up and no GLP-1RA use throughout follow up for the significant data by deterministically setting all exposure nodes A to 1 and 0, respectively, then re-simulating the data under each condition. For further detail, see Supplemental Materials 6. 

\subsubsection{Estimation procedure}

We considered both the inverse-probability of treatment weight (IPTW) estimator and targeted maximum-likelihood estimator (TMLE) as candidate estimators in the simulation. Longitudinal targeted maximum likelihood estimation (LTMLE)\cite{laan_targeted_2018,petersen_applying_2014} expands the targeted maximum likelihood estimator to a time-varying context. It is a double-robust plug-in estimator that enables researchers to control for time-dependent confounding that is affected by previous exposure without adjusting away the effect of the exposure on the outcome through downstream mediators. \cite{laan_targeted_2011,laan_targeted_2018} Nuisance parameters in LTMLE estimation can incorporate machine learning algorithms while maintaining statistically valid inference under met assupmtions.  However, both theory and prior empirical work demonstrate the vulnerability of this estimator to overfitting and the use of internal sample splits and cross-fititng (i.e. cv-TMLE) to address this problem.\cite{laan_targeted_2018} In the present case study, the lack of a computationally efficient implementation of this estimator for the longitudinal treatment effect of interest led us to instead rely on simulations to pre-specify an estimator expected to perform well despite challenges. 

We considered the following candidate algorithms for g and Q estimation: LASSO (CV-$\lambda$ minimum and one standard error from the minimum), Ridge, elastic net, generalized linear model (identity link, adjusted and unadjusted), and random forest. Due to rare events and high administrative censoring, we additionally considered estimation procedures with an intercept only model for Q estimation. 

As described above, incorporation of death as a competing event for dementia onset implies knowledge about the statistical model. In theory, by incorporating this knowledge in the estimation of the iterated outcome regression has the potential to reduce the variance of the estimator; however, the performance implications in complex finite sample data are less clear. We therefore examined estimator both with and without explicitly incorporating this knowledge (using the determinstic Q function in the ltmle package).\cite{gruber_tmle_2012} 

To estimate variance, we considered empirical influence curve variance, “robust” variance estimator \cite{tran_robust_2018}, and non-parametric bootstrap. To handle competing events, commonly, this information is incorporated into a censoring node. In our case, we are interested in death as a competing event. We examined estimates both with and without a deterministic function. Using a deterministic function,  we can set Q regression probabilities to 0 once a competing event, like death, has occurred.

We estimated the performance of each combination of the above specifications on 1000 datasets generated from our data generating process described above. To evaluate performance of the estimation procedures, we compared mean-squared error, bias, variance, bias to standard error ratio, coverage, and oracle coverage (Supplemental Materials 7). 

\subsection{Simulation and estimation selection}
We found that the TMLE estimator with LASSO nuisance parameter estimation, non-parametric bootstrap estimation and deterministic Q function. We found the non-parametric bootstrap to have coverage between the two built-in options in the \emph{ltmle} package. We found using a deterministic Q function to account for death as a competing risk did not change the estimate. For full simulation results, see Supplemental Materials 7.

\subsection{Analysis}
We then implemented the final analysis on the registry data. We additionally examined several pre-specified sensitivity analyses. We implemented the analysis using longer (12-month) and shorter (3-month) time intervals in order to assess the robustness of the results under differing levels of granularity. We restricted the data to later start years (2014 and later); this was to accommodate both the slower adoption of GLP-1RAs and later start of SGLT2 inhibitors, which came to market in 2014. 

For all analyses, we used R version 4.2, and the ltmle package.\cite{gruber_tmle_2012} 


\section{Results}


\subsection{Cohort demographics}

Of the historic diabetes patients using metformin in the registry and initiating second-line treatment between 2009 and 2021 (n=154,128), 104,928 met inclusion criteria and were included in the sample (Figure 1). 
\begin{figure}[H]
\includegraphics[width=\textwidth]{fig1.png}
\centering
\caption{Flowchart of selection criteria for retrospective cohort of diabetes patients initiating second line therapy for the first time between 2009 and 2021 in Denmark}
\end{figure}

Among those meeting inclusion criteria for the study, 13\% (n=13,334) began GLP-1RAs at baseline, and 87\% (n=91,594) began other second-line medications (for further detail on demographics of other treatment medication initiators, see Supplemental Materials 8). Those who began GLP-1RAs at index date were more likely to be below 55, to be more educated, have a higher income, and have a longer duration of diabetes (Table 2). Those initiating GLP-1RAs at baseline were more likely to have some conditions (chronic pulmonary disease), and less likely to have others (heart failure, renal disease, ischemic heart disease, myocardial infarction). Those initiating GLP-1RAs were more likely to be treated with Mineralocorticoid receptor antagonists (MRAs), Calcium channel blockers (CCBs), or Renin–angiotensin system inhibitors (RASIs).

By the end of the 5-year follow up, n=46,447 were censored (44\%). More patients were administratively censored in the treatment than the control group(70\% vs 41\%). There were n=27 cases of dementia among those who initiated GLP-1RA at baseline, and n=1819 cases of dementia among those initiating another second-line drug at baseline.

\newpage
\include{table1_new.tex}
\newpage
\subsection{Adjusted risk differences}

We plotted the marginal adjusted risk of dementia at each time point, among those who have survived until that time point and have followed the counterfactual treatment up until that time point. Adjusted results show a marked difference in the risk of dementia over time between the two counterfactual exposure groups (Figure 2;Table 3).
\newpage
\begin{landscape}
\newgeometry{left=3cm,bottom=0.1cm}
\begin{figure}[H]
\includegraphics[width=0.7\textwidth]{Fig2.png}
\centering
\caption{Adjusted marginal LTMLE dementia risk estimates comparing sustained treatment with GLP-1RAs and those not treated with GLP-1RAs at each 6-month follow up period in cohort of Danish second-line diabetes drug initiators 2009-2021}
\end{figure}
\begin{flushleft}
%\begin{tabular}
\input{table2_new}
%\end{tabular}
\end{flushleft}
\restoregeometry
\end{landscape}
\newpage
Adjusted results showed a protective effect comparing five-year continuous GLP-1RA use to continuous non-use (first target causal parameter). Null effects were found comparing GLP-1RAs to other active comparators, including any other second line, DPP4, or SGLT2 (Table 4).

\input{table3_results}

%\begin{figure}[H]
%\includegraphics[width=0.7\textwidth]{Fig3_grid.png}
%\centering
%\caption{Adjusted 5-year risk difference of dementia in a cohort of Danish diabetes patients initiating second-line therapy}
%\end{figure}
\subsection{Sensitivity analyses}
Results for the primary endpoint were attenuated when subset to 2014 start date (Table 5). Results were consistent when time unit discretization was changed to 12 months or to 3 months (Table 5). Shortening the time unit led to a wider confidence interval. 

\input{table_4.tex}


%\begin{figure}[H]
%\includegraphics[width=0.7\textwidth]{Fig4.png}
%\centering
%\caption{Sensitivity analyses for risk difference of dementia in a cohort of Danish diabetes patients initiating second-line therapy}
%\end{figure}


\section{Discussion}

In this study, we apply the casual roadmap to a longitudinal analysis of a large national registry database. Through the use of the roadmap, we explicitly state our causal parameter, assumptions required for causal inference, and distinguish between statistical and causal estimation. We found significant effects of GLP-1RAs on 5-year dementia risk compared to no usage of GLP-1RAs. Effects of GLP-1RAs compared to active comparator regimes were attenuated, likely due in part to decreased power. Comparison between GLP-1RA and SGLT2 inhibitors was particularly underpowered due to rare continuous usage of SGLT2 and more administrative censoring as SGLT2 is a newer drug (usage increasing after 2011). 

This finding agrees with prior literature on the benefit of GLP-1RAs on dementia onset in the Danish registry\cite{norgaard_treatment_2022} and some randomized \cite{vadini_liraglutide_2020, ballard_liraglutide_2020,cukierman-yaffe_effect_2020, gejl_alzheimers_2016} and observational studies \cite{onoviran_effects_2019,wium-andersen_antidiabetic_2019}. High administrative censoring of the treatment group is likely due to the relatively less common prescription of GLP-1RAs relative to other, more established second-line therapies.\cite{persson_different_2018}

In order to interpret the estimates causally, we would need to meet positivity and sequential randomization assumptions (i.e. have no unmeasured longitudinal confounding). Due to data availability, we were not able to adjust for smoking status or body mass index. This may lead to violations in the sequential randomization assumption and limit our causal interpretation of the effect estimate. In addition, while this sample is generalizable nationally to Denmark and to other Nordic countries, the ethnically homogeneous population in the Danish registry does not necessarily generalize to more diverse populations.  

Many researchers in observational settings choose not to conduct causal analyses due to perceived complexity. However, the step-wise nature of the causal roadmap lends itself to being easily followed. Following a roadmap ensures applied researchers to not fall into common traps, such as the causal interpretation of a statistical estimand without statement and evaluation of needed assumptions. 

To our knowledge, this is the first study of its kind of apply the longitudinal causal roadmap \cite{petersen_causal_2014, petersen_applying_2014} to a large national registry database. Through an applied example, we illustrate the importance of: defining a target causal parameter that clearly reflects one’s question of interest, stating needed assumptions and interpreting results in the context of the data and plausibility of assumptions. Crucially, we also demonstrate the desirability and feasibility of implementing a complex semi-paramteric efficient substitution estimator (L-TMLE) that integrates machine learning- despite the size and complexity of the dataset. Given the growing size and availability of health registry data, as well as its inherent limitations, it is paramount that causal analyses be implemented in a structured way that interprets results in context.


==> archive/old_table2.tex <==

\begin{adjustwidth}{-1in}{-1in}% adjust the L and R margins by 1 inch 
\noindent\setlength\tabcolsep{4pt}%
%\begin{table}[]
\begin{tabularx}{\linewidth}{|l|*{11}{>{\RaggedRight\arraybackslash}X|}}  \hline
%\begin{tabular}{llllllllllll}
                       & t=1         & t=2         & t=3         & t=4         & t=5         & t=6        & t=7        & t=8        & t=9        & t=10       & Total  \\
                         \hline
Total (n)                      &             &             &             &             &             &            &            &            &            &            & 104558 \\
Treatment GLP1         &             &             &             &             &             &            &            &            &            &            &        \\
\hline
Risk set at time t (n) & 13266       & 11176       & 9040        & 7518        & 6467        & 5732       & 4981       & 4479       & 4075       & 3763       &        \\
Dementia (n, \%)       & 8 (0.06)    & 3 (0.03)    & 2 (0.02)    & 2 (0.03)    & 2 (0.03)    & 1 (0.02)   & 5 (0.10)   & 2 (0.04)   & 1 (0.02)   & 1 (0.03)   & 27     \\
Death (n, \%)          & 94 (0.7)    & 81 (0.7)    & 62 (0.7)    & 58 (0.8)    & 46 (0.7)    & 40 (0.7)   & 36 (0.7)   & 46 (1.0)   & 43 (1.1)   & N/A        & 506    \\
Censored (n, \%)       & 1988 (15.0) & 2052 (18.4) & 1458 (16.1) & 991 (13.2)  & 687 (10.6)  & 710 (12.4) & 461 (9.3)  & 356 (7.9)  & 268 (6.6)  & 285 (7.6)  & 9256   \\
Control (no GLP1 use)  &             &             &             &             &             &            &            &            &            &            &        \\
\hline
Risk set at time t (n) & 91292       & 86777       & 79845       & 74362       & 69167       & 64632      & 59765      & 55633      & 51146      & 47248      &        \\
Dementia (n, \%)       & 113 (0.9)   & 226 (2.0)   & 212 (2.3)   & 199 (2.6)   & 210 (3.2)   & 199 (3.5)  & 177 (3.6)  & 166 (3.7)  & 157 (3.9)  & 160 (4.3)  & 1819   \\
Death (n, \%)          & 1704 (12.8) & 1343 (12.0) & 1235 (13.7) & 1118 (14.9) & 1081 (16.7) & 973 (17.0) & 956 (19.2) & 923 (20.6) & 875 (21.5) & N/A        & 10208  \\
Censored (n, \%)       & 4515 (4.9)  & 5115 (5.9)  & 4027 (5.0)  & 3861 (5.2)  & 3317 (4.8)  & 3676 (5.7) & 3070 (5.1) & 3443 (6.2) & 2897 (5.7) & 3270 (6.9) & 37191 \\
\hline
\end{tabularx}
\captionof{table}{Table of longitudinal patterns in treatment and control groups in a cohort of diabetes patients initiating second line use between 2009 and 2021 in Denmark}

%\end{center}
\end{adjustwidth}


==> archive/table2_archive.tex <==

%\begin{adjustwidth}{-1in}{-1in}% adjust the L and R margins by 1 inch 
\noindent\setlength\tabcolsep{4pt}%
%\begin{tabular}[]
\begin{tabularx}{\linewidth}{|l|*{11}{>{\RaggedRight\arraybackslash}X|}}  \hline
%\begin{tabular}{llllllllllll}
                       & t=1         & t=2         & t=3         & t=4         & t=5         & t=6        & t=7        & t=8        & t=9        & t=10       &   \\
                         \hline
Total (n)                      &             &             &             &             &             &            &            &            &            &            & 104558 \\
\hline
Treatment GLP1         &             &             &             &             &             &            &            &            &            &            &        \\

Risk set at time t (n) & 13266       & 11176       & 9040        & 7518        & 6467        & 5732       & 4981       & 4479       & 4075       & 3763       &        \\
\hline

Control (no GLP1 use)  &             &             &             &             &             &            &            &            &            &            &        \\
Risk set at time t (n) & 91292       & 86777       & 79845       & 74362       & 69167       & 64632      & 59765      & 55633      & 51146      & 47248      &        \\

\hline
\end{tabularx}
\captionof{table}{Table of longitudinal patterns in treatment and control groups in a cohort of diabetes patients initiating second line use between 2009 and 2021 in Denmark}
%\end{tabular}
%\end{center}
%\end{adjustwidth}


==> archive/table3_new.tex <==
% \usepackage{tabularray}
\begin{table}[!ht]
\centering
\resizebox{\linewidth}{!}{%
\begin{tblr}{
  width =  \linewidth,
  colspec = {Q[267]Q[194]Q[157]Q[319]},
  column{even} = {l},
  column{3} = {l},
  hline{2} = {-}{-},
}
Comparison          & Treatment Risk & Control Risk & Risk Difference (95\% CI) \\
\hline
1) GLP1 vs. no GLP1 & 0.0069         & 0.0133       & -0.0064 (-0.0085,-0.0043) \\
2) GLP1 vs. SGLT2   & 0.0071         & 0.0074       & -0.0003 (-0.0027,0.0022)  \\
3) GLP1 vs. DPP4    & 0.0068         & 0.0115       & -0.0048 (-0.0093,-0.0002)    
\end{tblr}
}
\caption{Adjusted 5-year risk difference of dementia in a cohort of Danish diabetes patients initiating second-line therapy}
\end{table}

==> r_citation.tex <==
@Manual{r_package,
    title = {R: A Language and Environment for Statistical Computing},
    author = {{R Core Team}},
    organization = {R Foundation for Statistical Computing},
    address = {Vienna, Austria},
    year = {2022},
    url = {https://www.R-project.org/},
  }
